PerfectDou: Dominating DouDizhu with Perfect Information Distillation

As a challenging multi-player card game, DouDizhu has recently drawn much attention for analyzing competition and collaboration in imperfect-information games. In this paper, we propose PerfectDou, a state-of-the-art DouDizhu AI system that dominates the game, in an actor-critic framework with a proposed technique named perfect information distillation. In detail, we adopt a perfect-training-imperfect-execution framework that allows the agents to utilize the global information to guide the training of the policies as if it is a perfect information game and the trained policies can be used to play the imperfect information game during the actual gameplay. To this end, we characterize card and game features for DouDizhu to represent the perfect and imperfect information. To train our system, we adopt proximal policy optimization with generalized advantage estimation in a parallel training paradigm. In experiments we show how and why PerfectDou beats all existing AI programs, and achieves state-of-the-art performance.

==> papers/7-1-action-space.tex <==
\begin{lstlisting}[title={Detailed Discrete Action Space (\texttt{"card combination" : action ID}, ~~~"*" can represent any card)}, frame=shadowbox]
{
    "3": 0,
    "4": 1,
    "5": 2,
    "6": 3,
    "7": 4,
    "8": 5,
    "9": 6,
    "T": 7,
    "J": 8,
    "Q": 9,
    "K": 10,
    "A": 11,
    "2": 12,
    "B": 13,
    "R": 14,
    "33": 15,
    "44": 16,
    "55": 17,
    "66": 18,
    "77": 19,
    "88": 20,
    "99": 21,
    "TT": 22,
    "JJ": 23,
    "QQ": 24,
    "KK": 25,
    "AA": 26,
    "22": 27,
    "333": 28,
    "444": 29,
    "555": 30,
    "666": 31,
    "777": 32,
    "888": 33,
    "999": 34,
    "TTT": 35,
    "JJJ": 36,
    "QQQ": 37,
    "KKK": 38,
    "AAA": 39,
    "222": 40,
    "3334": 41,
    "3335": 42,
    "3336": 43,
    "3337": 44,
    "3338": 45,
    "3339": 46,
    "333T": 47,
    "333J": 48,
    "333Q": 49,
    "333K": 50,
    "333A": 51,
    "3332": 52,
    "333B": 53,
    "333R": 54,
    "3444": 55,
    "4445": 56,
    "4446": 57,
    "4447": 58,
    "4448": 59,
    "4449": 60,
    "444T": 61,
    "444J": 62,
    "444Q": 63,
    "444K": 64,
    "444A": 65,
    "4442": 66,
    "444B": 67,
    "444R": 68,
    "3555": 69,
    "4555": 70,
    "5556": 71,
    "5557": 72,
    "5558": 73,
    "5559": 74,
    "555T": 75,
    "555J": 76,
    "555Q": 77,
    "555K": 78,
    "555A": 79,
    "5552": 80,
    "555B": 81,
    "555R": 82,
    "3666": 83,
    "4666": 84,
    "5666": 85,
    "6667": 86,
    "6668": 87,
    "6669": 88,
    "666T": 89,
    "666J": 90,
    "666Q": 91,
    "666K": 92,
    "666A": 93,
    "6662": 94,
    "666B": 95,
    "666R": 96,
    "3777": 97,
    "4777": 98,
    "5777": 99,
    "6777": 100,
    "7778": 101,
    "7779": 102,
    "777T": 103,
    "777J": 104,
    "777Q": 105,
    "777K": 106,
    "777A": 107,
    "7772": 108,
    "777B": 109,
    "777R": 110,
    "3888": 111,
    "4888": 112,
    "5888": 113,
    "6888": 114,
    "7888": 115,
    "8889": 116,
    "888T": 117,
    "888J": 118,
    "888Q": 119,
    "888K": 120,
    "888A": 121,
    "8882": 122,
    "888B": 123,
    "888R": 124,
    "3999": 125,
    "4999": 126,
    "5999": 127,
    "6999": 128,
    "7999": 129,
    "8999": 130,
    "999T": 131,
    "999J": 132,
    "999Q": 133,
    "999K": 134,
    "999A": 135,
    "9992": 136,
    "999B": 137,
    "999R": 138,
    "3TTT": 139,
    "4TTT": 140,
    "5TTT": 141,
    "6TTT": 142,
    "7TTT": 143,
    "8TTT": 144,
    "9TTT": 145,
    "TTTJ": 146,
    "TTTQ": 147,
    "TTTK": 148,
    "TTTA": 149,
    "TTT2": 150,
    "TTTB": 151,
    "TTTR": 152,
    "3JJJ": 153,
    "4JJJ": 154,
    "5JJJ": 155,
    "6JJJ": 156,
    "7JJJ": 157,
    "8JJJ": 158,
    "9JJJ": 159,
    "TJJJ": 160,
    "JJJQ": 161,
    "JJJK": 162,
    "JJJA": 163,
    "JJJ2": 164,
    "JJJB": 165,
    "JJJR": 166,
    "3QQQ": 167,
    "4QQQ": 168,
    "5QQQ": 169,
    "6QQQ": 170,
    "7QQQ": 171,
    "8QQQ": 172,
    "9QQQ": 173,
    "TQQQ": 174,
    "JQQQ": 175,
    "QQQK": 176,
    "QQQA": 177,
    "QQQ2": 178,
    "QQQB": 179,
    "QQQR": 180,
    "3KKK": 181,
    "4KKK": 182,
    "5KKK": 183,
    "6KKK": 184,
    "7KKK": 185,
    "8KKK": 186,
    "9KKK": 187,
    "TKKK": 188,
    "JKKK": 189,
    "QKKK": 190,
    "KKKA": 191,
    "KKK2": 192,
    "KKKB": 193,
    "KKKR": 194,
    "3AAA": 195,
    "4AAA": 196,
    "5AAA": 197,
    "6AAA": 198,
    "7AAA": 199,
    "8AAA": 200,
    "9AAA": 201,
    "TAAA": 202,
    "JAAA": 203,
    "QAAA": 204,
    "KAAA": 205,
    "AAA2": 206,
    "AAAB": 207,
    "AAAR": 208,
    "3222": 209,
    "4222": 210,
    "5222": 211,
    "6222": 212,
    "7222": 213,
    "8222": 214,
    "9222": 215,
    "T222": 216,
    "J222": 217,
    "Q222": 218,
    "K222": 219,
    "A222": 220,
    "222B": 221,
    "222R": 222,
    "33344": 223,
    "33355": 224,
    "33366": 225,
    "33377": 226,
    "33388": 227,
    "33399": 228,
    "333TT": 229,
    "333JJ": 230,
    "333QQ": 231,
    "333KK": 232,
    "333AA": 233,
    "33322": 234,
    "33444": 235,
    "44455": 236,
    "44466": 237,
    "44477": 238,
    "44488": 239,
    "44499": 240,
    "444TT": 241,
    "444JJ": 242,
    "444QQ": 243,
    "444KK": 244,
    "444AA": 245,
    "44422": 246,
    "33555": 247,
    "44555": 248,
    "55566": 249,
    "55577": 250,
    "55588": 251,
    "55599": 252,
    "555TT": 253,
    "555JJ": 254,
    "555QQ": 255,
    "555KK": 256,
    "555AA": 257,
    "55522": 258,
    "33666": 259,
    "44666": 260,
    "55666": 261,
    "66677": 262,
    "66688": 263,
    "66699": 264,
    "666TT": 265,
    "666JJ": 266,
    "666QQ": 267,
    "666KK": 268,
    "666AA": 269,
    "66622": 270,
    "33777": 271,
    "44777": 272,
    "55777": 273,
    "66777": 274,
    "77788": 275,
    "77799": 276,
    "777TT": 277,
    "777JJ": 278,
    "777QQ": 279,
    "777KK": 280,
    "777AA": 281,
    "77722": 282,
    "33888": 283,
    "44888": 284,
    "55888": 285,
    "66888": 286,
    "77888": 287,
    "88899": 288,
    "888TT": 289,
    "888JJ": 290,
    "888QQ": 291,
    "888KK": 292,
    "888AA": 293,
    "88822": 294,
    "33999": 295,
    "44999": 296,
    "55999": 297,
    "66999": 298,
    "77999": 299,
    "88999": 300,
    "999TT": 301,
    "999JJ": 302,
    "999QQ": 303,
    "999KK": 304,
    "999AA": 305,
    "99922": 306,
    "33TTT": 307,
    "44TTT": 308,
    "55TTT": 309,
    "66TTT": 310,
    "77TTT": 311,
    "88TTT": 312,
    "99TTT": 313,
    "TTTJJ": 314,
    "TTTQQ": 315,
    "TTTKK": 316,
    "TTTAA": 317,
    "TTT22": 318,
    "33JJJ": 319,
    "44JJJ": 320,
    "55JJJ": 321,
    "66JJJ": 322,
    "77JJJ": 323,
    "88JJJ": 324,
    "99JJJ": 325,
    "TTJJJ": 326,
    "JJJQQ": 327,
    "JJJKK": 328,
    "JJJAA": 329,
    "JJJ22": 330,
    "33QQQ": 331,
    "44QQQ": 332,
    "55QQQ": 333,
    "66QQQ": 334,
    "77QQQ": 335,
    "88QQQ": 336,
    "99QQQ": 337,
    "TTQQQ": 338,
    "JJQQQ": 339,
    "QQQKK": 340,
    "QQQAA": 341,
    "QQQ22": 342,
    "33KKK": 343,
    "44KKK": 344,
    "55KKK": 345,
    "66KKK": 346,
    "77KKK": 347,
    "88KKK": 348,
    "99KKK": 349,
    "TTKKK": 350,
    "JJKKK": 351,
    "QQKKK": 352,
    "KKKAA": 353,
    "KKK22": 354,
    "33AAA": 355,
    "44AAA": 356,
    "55AAA": 357,
    "66AAA": 358,
    "77AAA": 359,
    "88AAA": 360,
    "99AAA": 361,
    "TTAAA": 362,
    "JJAAA": 363,
    "QQAAA": 364,
    "KKAAA": 365,
    "AAA22": 366,
    "33222": 367,
    "44222": 368,
    "55222": 369,
    "66222": 370,
    "77222": 371,
    "88222": 372,
    "99222": 373,
    "TT222": 374,
    "JJ222": 375,
    "QQ222": 376,
    "KK222": 377,
    "AA222": 378,
    "34567": 379,
    "45678": 380,
    "56789": 381,
    "6789T": 382,
    "789TJ": 383,
    "89TJQ": 384,
    "9TJQK": 385,
    "TJQKA": 386,
    "345678": 387,
    "456789": 388,
    "56789T": 389,
    "6789TJ": 390,
    "789TJQ": 391,
    "89TJQK": 392,
    "9TJQKA": 393,
    "3456789": 394,
    "456789T": 395,
    "56789TJ": 396,
    "6789TJQ": 397,
    "789TJQK": 398,
    "89TJQKA": 399,
    "3456789T": 400,
    "456789TJ": 401,
    "56789TJQ": 402,
    "6789TJQK": 403,
    "789TJQKA": 404,
    "3456789TJ": 405,
    "456789TJQ": 406,
    "56789TJQK": 407,
    "6789TJQKA": 408,
    "3456789TJQ": 409,
    "456789TJQK": 410,
    "56789TJQKA": 411,
    "3456789TJQK": 412,
    "456789TJQKA": 413,
    "3456789TJQKA": 414,
    "334455": 415,
    "445566": 416,
    "556677": 417,
    "667788": 418,
    "778899": 419,
    "8899TT": 420,
    "99TTJJ": 421,
    "TTJJQQ": 422,
    "JJQQKK": 423,
    "QQKKAA": 424,
    "33445566": 425,
    "44556677": 426,
    "55667788": 427,
    "66778899": 428,
    "778899TT": 429,
    "8899TTJJ": 430,
    "99TTJJQQ": 431,
    "TTJJQQKK": 432,
    "JJQQKKAA": 433,
    "3344556677": 434,
    "4455667788": 435,
    "5566778899": 436,
    "66778899TT": 437,
    "778899TTJJ": 438,
    "8899TTJJQQ": 439,
    "99TTJJQQKK": 440,
    "TTJJQQKKAA": 441,
    "334455667788": 442,
    "445566778899": 443,
    "5566778899TT": 444,
    "66778899TTJJ": 445,
    "778899TTJJQQ": 446,
    "8899TTJJQQKK": 447,
    "99TTJJQQKKAA": 448,
    "33445566778899": 449,
    "445566778899TT": 450,
    "5566778899TTJJ": 451,
    "66778899TTJJQQ": 452,
    "778899TTJJQQKK": 453,
    "8899TTJJQQKKAA": 454,
    "33445566778899TT": 455,
    "445566778899TTJJ": 456,
    "5566778899TTJJQQ": 457,
    "66778899TTJJQQKK": 458,
    "778899TTJJQQKKAA": 459,
    "33445566778899TTJJ": 460,
    "445566778899TTJJQQ": 461,
    "5566778899TTJJQQKK": 462,
    "66778899TTJJQQKKAA": 463,
    "33445566778899TTJJQQ": 464,
    "445566778899TTJJQQKK": 465,
    "5566778899TTJJQQKKAA": 466,
    "333444": 467,
    "444555": 468,
    "555666": 469,
    "666777": 470,
    "777888": 471,
    "888999": 472,
    "999TTT": 473,
    "TTTJJJ": 474,
    "JJJQQQ": 475,
    "QQQKKK": 476,
    "KKKAAA": 477,
    "333444555": 478,
    "444555666": 479,
    "555666777": 480,
    "666777888": 481,
    "777888999": 482,
    "888999TTT": 483,
    "999TTTJJJ": 484,
    "TTTJJJQQQ": 485,
    "JJJQQQKKK": 486,
    "QQQKKKAAA": 487,
    "333444555666": 488,
    "444555666777": 489,
    "555666777888": 490,
    "666777888999": 491,
    "777888999TTT": 492,
    "888999TTTJJJ": 493,
    "999TTTJJJQQQ": 494,
    "TTTJJJQQQKKK": 495,
    "JJJQQQKKKAAA": 496,
    "333444555666777": 497,
    "444555666777888": 498,
    "555666777888999": 499,
    "666777888999TTT": 500,
    "777888999TTTJJJ": 501,
    "888999TTTJJJQQQ": 502,
    "999TTTJJJQQQKKK": 503,
    "TTTJJJQQQKKKAAA": 504,
    "333444555666777888": 505,
    "444555666777888999": 506,
    "555666777888999TTT": 507,
    "666777888999TTTJJJ": 508,
    "777888999TTTJJJQQQ": 509,
    "888999TTTJJJQQQKKK": 510,
    "999TTTJJJQQQKKKAAA": 511,
    "333444**": 512,
    "444555**": 513,
    "555666**": 514,
    "666777**": 515,
    "777888**": 516,
    "888999**": 517,
    "999TTT**": 518,
    "TTTJJJ**": 519,
    "JJJQQQ**": 520,
    "QQQKKK**": 521,
    "KKKAAA**": 522,
    "333444555***": 523,
    "444555666***": 524,
    "555666777***": 525,
    "666777888***": 526,
    "777888999***": 527,
    "888999TTT***": 528,
    "999TTTJJJ***": 529,
    "TTTJJJQQQ***": 530,
    "JJJQQQKKK***": 531,
    "QQQKKKAAA***": 532,
    "333444555666****": 533,
    "444555666777****": 534,
    "555666777888****": 535,
    "666777888999****": 536,
    "777888999TTT****": 537,
    "888999TTTJJJ****": 538,
    "999TTTJJJQQQ****": 539,
    "TTTJJJQQQKKK****": 540,
    "JJJQQQKKKAAA****": 541,
    "333444555666777*****": 542,
    "444555666777888*****": 543,
    "555666777888999*****": 544,
    "666777888999TTT*****": 545,
    "777888999TTTJJJ*****": 546,
    "888999TTTJJJQQQ*****": 547,
    "999TTTJJJQQQKKK*****": 548,
    "TTTJJJQQQKKKAAA*****": 549,
    "333444****": 550,
    "444555****": 551,
    "555666****": 552,
    "666777****": 553,
    "777888****": 554,
    "888999****": 555,
    "999TTT****": 556,
    "TTTJJJ****": 557,
    "JJJQQQ****": 558,
    "QQQKKK****": 559,
    "KKKAAA****": 560,
    "333444555******": 561,
    "444555666******": 562,
    "555666777******": 563,
    "666777888******": 564,
    "777888999******": 565,
    "888999TTT******": 566,
    "999TTTJJJ******": 567,
    "TTTJJJQQQ******": 568,
    "JJJQQQKKK******": 569,
    "QQQKKKAAA******": 570,
    "333444555666********": 571,
    "444555666777********": 572,
    "555666777888********": 573,
    "666777888999********": 574,
    "777888999TTT********": 575,
    "888999TTTJJJ********": 576,
    "999TTTJJJQQQ********": 577,
    "TTTJJJQQQKKK********": 578,
    "JJJQQQKKKAAA********": 579,
    "3333**": 580,
    "4444**": 581,
    "5555**": 582,
    "6666**": 583,
    "7777**": 584,
    "8888**": 585,
    "9999**": 586,
    "TTTT**": 587,
    "JJJJ**": 588,
    "QQQQ**": 589,
    "KKKK**": 590,
    "AAAA**": 591,
    "2222**": 592,
    "3333****": 593,
    "4444****": 594,
    "5555****": 595,
    "6666****": 596,
    "7777****": 597,
    "8888****": 598,
    "9999****": 599,
    "TTTT****": 600,
    "JJJJ****": 601,
    "QQQQ****": 602,
    "KKKK****": 603,
    "AAAA****": 604,
    "2222****": 605,
    "3333": 606,
    "4444": 607,
    "5555": 608,
    "6666": 609,
    "7777": 610,
    "8888": 611,
    "9999": 612,
    "TTTT": 613,
    "JJJJ": 614,
    "QQQQ": 615,
    "KKKK": 616,
    "AAAA": 617,
    "2222": 618,
    "BR": 619,
    "pass": 620
}
\end{lstlisting}

==> papers/8-checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerNo{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We include data, implementation details for reproduction. See \ap{ap:exps}. But the codes have not been public for now.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We try to cover all the training details. See \ap{ap:exps}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{We do not do that simply following the convention of previous works.}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See \ap{ap:exps}}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See \se{sec:exps}.}
  \item Did you mention the license of the assets?
    \answerNo{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See \se{sec:exps}}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}
